Outer Rotation Curve of the Galaxy with VERA III: Astrometry of IRAS 07427-2400 and Test of the Density-Wave Theory

We report the trigonometric parallax of IRAS 07427-2400 with VERA to be 0.185 $\pm$ 0.027 mas, corresponding to a distance of 5.41$^{+0.92}_{-0.69}$ kpc. The result is consistent with the previous result of 5.32$^{+0.49}_{-0.42}$ kpc obtained by Choi et al. (2014) within error. To remove the effect of internal maser motions (e.g., random motions), we observed six maser features associated with IRAS 07427-2400 and determined systematic proper motions of the source by averaging proper motions of the six maser features. The obtained proper motions are ($\mu_{\alpha}$cos$\delta$, $\mu_{\delta}$) = ($-$1.79 $\pm$ 0.32, 2.60 $\pm$ 0.17) mas yr$^{-1}$ in equatorial coordinates, while Choi et al. (2014) showed ($\mu_{\alpha}$cos$\delta$, $\mu_{\delta}$) = ($-$2.43 $\pm$ 0.02, 2.49 $\pm$ 0.09) mas yr$^{-1}$ with one maser feature. Our astrometry results place the source in the Perseus arm, the nearest main arm in the Milky Way. Using our result with previous astrometry results obtained from observations of the Perseus arm, we conducted direct (quantitative) comparisons between 27 astrometry results and an analytic gas dynamics model based on the density-wave theory and obtained two results. First is the pitch angle of the Perseus arm determined by VLBI astrometry, 11.1 $\pm$ 1.4 deg, differing from what is determined by the spiral potential model (probably traced by stars), $\sim$ 20 deg. The second is an offset between a dense gas region and the bottom of the spiral potential model. The dense gas region traced by VLBI astrometry is located downstream of the spiral potential model, which was previously confirmed in the nearby grand-design spiral galaxy M51 in Egusa et al. (2011).

==> 00README.XXX.tex <==
nohypertex

